ABAMGuid+: An Enhanced Aerocapture Guidance Framework using Augmented Bank Angle Modulation

Aerocapture consists of converting a hyperbolic approach trajectory into a captured target orbit utilizing the aerodynamic forces generated via a single pass through the atmosphere. Aerocapture guidance systems must be robust to significant environmental variations and modeling uncertainty, particularly regarding atmospheric properties and delivery conditions. Recent work has shown that enabling control over both bank angle and angle of attack, a strategy referred to as augmented bank angle modulation (ABAM), can improve robustness to entry state and atmospheric uncertainties. In this work, we derive optimal control solutions for an aerocapture vehicle using ABAM. We first formulate the problem using a linear aerodynamic model and derive closed-form optimal control profiles using Pontryagin's Minimum Principle. To increase modeling fidelity, we also consider a quadratic aerodynamic model and obtain the solution directly using the optimality conditions. Both formulations are solved numerically using Gauss pseudospectral methods (via GPOPS, a software tool for pseudospectral optimal control), to validate the analytic solutions. We then introduce a novel aerocapture guidance algorithm, ABAMGuid+, which indirectly minimizes propellant usage by mimicking the structure of the optimal control solution, enabling efficient guidance by avoiding the complexity of solving the full optimal control problem online. Extensive Monte Carlo simulations of a Uranus aerocapture mission demonstrate that ABAMGuid+ increases capture success rates and reduces post-capture propellant requirements relative to previous methods.

==> Aerodynamic_Modeling.tex <==
Aerodynamic properties are modeled in simulation via CFD analysis in \cite{shellabarger2025aerodynamics} and stored in lookup tables as nonlinear functions of angle of attack. To obtain an analytic solution for the optimal control profiles, a functional approximation on the form of $C_D(\alpha)$ and $C_L(\alpha)$ is necessary. In this work, we consider linear and quadratic aerodynamic models.
The linear model assumes that the lift and drag coefficients vary linearly as a function of angle of attack as 
\begin{equation} \label{eq: linear aero model}
C_D(\alpha) = C_{D_\alpha} \alpha + C_{D,0}, \quad
C_L(\alpha) = C_{L_\alpha} \alpha + C_{L,0}.
\end{equation}
The quadratic model is given by  
\begin{equation}  \label{eq: quadratic aero model}
C_D(\alpha) = C_{D, \alpha^2} \alpha^2 + C_{D, \alpha} \alpha + C_{D,0}, \quad
C_L(\alpha) = C_{L, \alpha^2} \alpha^2 + C_{L, \alpha} \alpha + C_{L,0}.
\end{equation}
Figure \ref{Aero Fits} shows the linear (blue) and quadratic (black) drag models (left panel) resulting from fitting the nonlinear aerodynamic database used in simulation to a linear and quadratic function of $\alpha$, as well as the error percentage compared to truth (right panel). The nonlinear aerodynamic model is given in red for comparison. The coefficients are given in Table \ref{tab:aeroCoeffs}. In the right panel, the black dashed lines represent $\pm$ 3\% error for reference.
We observe that when $\alpha$ $\in$ [-10, -25], the linearly approximated $D$ error percentage is within 3\% for the entire range, suggesting that the linear model is a reasonable approximation of the true aerodynamics within this range. Previous work \cite{deshmukh2020investigation} has shown that this level of accuracy is well within the valid range for blunt bodied aerocapture vehicles. For the quadratic model over the same range, the error percentage drops to within $\approx$ 0.3\%, indicating that the quadratic model is extremely close to the true aerodynamics. 
The lift model follows a similar trend, and thus is omitted from the analysis.

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.8\textwidth]{CD_combined.eps}
	\caption{Linear (blue) and quadratic (black) $C_D$ approximations versus true aerodynamics (red) as a function of angle of attack (left panel). The right panel displays error percentage versus truth over the $\alpha$ range. The linear model well approximates the true nonlinear aerodynamics, and the quadratic model is nearly identical to truth.} \label{Aero Fits}
\end{figure}

\begin{table}[htbp] 
\centering
\caption{Aerodynamic coefficients for linear and quadratic models.}
\label{tab:aeroCoeffs}
\begin{tabular}{lcc}
\toprule
\toprule
\textbf{Coefficient} & \textbf{Linear Model} & \textbf{Quadratic Model} \\
\midrule
\(C_{D, 0}\) & 1.72 & 1.59 \\
\(C_{L, 0}\) & $7.07 \cdot 10^{-2}$ & $-2.71 \cdot 10^{-2}$ \\
\(C_{D, \alpha}\) & $1.87 \cdot 10^{-2}$ & $3.83 \cdot 10^{-3}$ \\
\(C_{L, \alpha}\) &$ -1.62 \cdot 10^{-2}$ &$ -2.82 \cdot 10^{-2}$ \\
\(C_{D, \alpha^2}\) & -- & $-4.25 \cdot 10^{-4} $\\
\(C_{L, \alpha^2}\) & -- & $-3.43 \cdot 10^{-4} $\\
\bottomrule
\bottomrule
\end{tabular}
\end{table}

